On Finding Randomly Planted Cliques in Arbitrary Graphs

We study a planted clique model introduced by Feige where a complete graph of size $c\cdot n$ is planted uniformly at random in an arbitrary $n$-vertex graph. We give a simple deterministic algorithm that, in almost linear time, recovers a clique of size $(c/3)^{O(1/c)} \cdot n$ as long as the original graph has maximum degree at most $(1-p)n$ for some fixed $p>0$. The proof hinges on showing that the degrees of the final graph are correlated with the planted clique, in a way similar to (but more intricate than) the classical $G(n,\frac{1}{2})+K_{\sqrt{n}}$ planted clique model. Our algorithm suggests a separation from the worst-case model, where, assuming the Unique Games Conjecture, no polynomial algorithm can find cliques of size $\Omega(n)$ for every fixed $c>0$, even if the input graph has maximum degree $(1-p)n$. Our techniques extend beyond the planted clique model. For example, when the planted graph is a balanced biclique, we recover a balanced biclique of size larger than the best guarantees known for the worst case.

==> macros.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{observation}{Observation}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}

\newcommand{\poly}{\operatorname{poly}}

\newcommand{\scG}{\mathcal{G}}
\newcommand{\scC}{\mathcal{C}}
\newcommand{\scA}{\mathcal{A}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\pr}{\operatorname{Pr}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\AlgoName}[1]{\ensuremath{\textsc{#1}}}

\newcommand{\DenseCliqueFinder}{\AlgoName{DenseCliqueFinder}}
\newcommand{\CliqueFinder}{\AlgoName{CliqueFinder}}
\newcommand{\BalancedBicliqueFinder}{\AlgoName{BalancedBicliqueFinder}}


